Backdoor Attacks Against Deep Learning Systems in the Physical World

Backdoor attacks embed hidden malicious behaviors into deep learning models, which only activate and cause misclassifications on model inputs containing a specific trigger. Existing works on backdoor attacks and defenses, however, mostly focus on digital attacks that use digitally generated patterns as triggers. A critical question remains unanswered: can backdoor attacks succeed using physical objects as triggers, thus making them a credible threat against deep learning systems in the real world? We conduct a detailed empirical study to explore this question for facial recognition, a critical deep learning task. Using seven physical objects as triggers, we collect a custom dataset of 3205 images of ten volunteers and use it to study the feasibility of physical backdoor attacks under a variety of real-world conditions. Our study reveals two key findings. First, physical backdoor attacks can be highly successful if they are carefully configured to overcome the constraints imposed by physical objects. In particular, the placement of successful triggers is largely constrained by the target model's dependence on key facial features. Second, four of today's state-of-the-art defenses against (digital) backdoors are ineffective against physical backdoors, because the use of physical objects breaks core assumptions used to construct these defenses. Our study confirms that (physical) backdoor attacks are not a hypothetical phenomenon but rather pose a serious real-world threat to critical classification tasks. We need new and more robust defenses against backdoors in the physical world.

==> Makefile <==
LATEX=latex
BIBTEX=bibtex

PAPER= realbackdoor
SUBMIT= backdoor-submit
SUPP=supplementary

BIBFILE=realbackdoor.bib translearn.bib
SUPPTEXFILES = supplementary.tex
TEXFILES = realbackdoor.tex \
	intro_cvpr.tex \
	back_cvpr.tex \
	method_cvpr.tex \
	experiment.tex \
	eval_cvpr.tex \
	realworld_cvpr.tex \
	advanced_cvpr.tex \
	countermeasure_cvpr.tex \
	conclusion_cvpr.tex \
	appendix_cvpr.tex \
	acknowledgements.tex


EPSFIGS = \

EPSGRAPHS = $(wildcard figs/*.eps)

all:   $(PAPER).pdf

submit:   $(SUBMIT).pdf

supp: $(SUPP).pdf

subdirs:
	$(MAKE) -C figs

bib:
	$(BIBTEX) (PAPER)

%.eps: %.plt

%.eps: %.fig
	fig2dev -L eps $< $@

$(PAPER).ps: $(PAPER).dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(PAPER).dvi > $(PAPER).ps

$(PAPER).pdf: $(PAPER).dvi
	dvipdf $(PAPER).dvi

# if need to embed font
$(SUBMIT).pdf: $(PAPER).ps
	ps2pdf14 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(PAPER).ps $(SUBMIT).pdf

$(PAPER).dvi: $(EPSFIGS) $(TEXFILES) $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

# For the supplementary
$(SUPP).dvi: $(EPSFIGS) $(SUPPTEXFILES) $(BIBFILE)
	$(LATEX)  $(SUPP)
	$(BIBTEX) $(SUPP)
	$(LATEX) $(SUPP)
	$(LATEX)  $(SUPP)

$(SUPP).blg: $(BIBFILE)
	$(LATEX)  $(SUPP)
	$(BIBTEX) $(SUPP)
	$(LATEX)  $(SUPP)

$(SUPP).ps: $(SUPP).dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(SUPP).dvi > $(SUPP).ps

$(SUPP).pdf: $(SUPP).dvi
	dvipdf $(SUPP).dvi


clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out


==> header.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{appendix}
\usepackage{comment}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{booktabs}
\usepackage{nicefrac}
%\usepackage{cryptocode}
\usepackage{tikz}
\usetikzlibrary{patterns}
%\usepackage{crypto-environments}
%\usepackage{nicodemus}
\usepackage{setspace}\usepackage{setspace}

\newcommand{\heading}[1]{\vspace{5pt}\noindent\textbf{{#1}}}

\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}
\newcommand{\Hrule}{\rule{\linewidth}{0.3mm}}

\newcommand{\scalefactor}{0.9}

\DeclareMathOperator*{\argmin}{arg\,min}


\newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{conjecture}{Conjecture}
\newtheorem{lemma}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{conj}{Conjecture}
\newcommand{\Vol}{\textsf{Vol}}

%\usepackage[dvipsnames]{xcolor}
\usepackage{epsfig,endnotes}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{url}
\usepackage{multirow}
\usepackage{bbding}
\usepackage{adjustbox}
\usepackage{times}
\usepackage{balance}
\usepackage{diagbox} 
\usepackage[pagebackref=true,colorlinks,bookmarks=false,hypertexnames=false]{hyperref}
\usepackage{hyperref}
\usepackage[hyphenbreaks]{breakurl}
%\usepackage{algorithm}
%\usepackage[noend]{algpseudocode}
\usepackage{subfigure}
\usepackage{tablefootnote}
\usepackage{booktabs}
\usepackage{bbm}
\usepackage{graphicx}
\usepackage{caption}\usepackage{array}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{53}}%

\newcolumntype{?}{!{\vrule width 1pt}}

\newcommand{\para}[1]{{\vspace{2pt} \bf \noindent #1 \hspace{2pt}}}
\newcommand\note[1]{{\em\color{black} #1}}
\newcommand\emily[1]{{\color{black} #1}}
\newcommand\ejw[1]{{\color{black} #1}}
%\newcommand\todo[1]{{\color{red} {\bf TODO:} #1}}
\newcommand\jos[1]{{\color{teal} {\bf Josephine:} #1}}
\newcommand\htedit[1]{{\color{black} #1}}
\newcommand\kedit[1]{{\color{black} #1}}
\newcommand\abedit[1]{{\color{black} #1}}
\newcommand\ab[1]{{\color{black} (ANB: #1)}}

% Actual editing commands to use!!
\newcommand\todo[1]{{\color{black} {\bf TODO:} #1}}
\newcommand\fixme[1]{{\bf \color{magenta} [#1]}}
\newcommand\edit[1]{{\color{teal} #1}}
%\newcommand\edit[1]{{\color{black} #1}}

%\newcommand\todo[1]{{\color{Red} {\bf TODO:} #1}}
%\newcommand\fixme[1]{{\bf \color{magenta} [#1]}}
%\newcommand\edit[1]{{\color{teal} #1}}

\newcommand{\model}{{\mathcal{F}_{\theta}}}
% \newcommand{\secspace}{\vspace{-0.12in}}
\newcommand{\secspace}{\vspace{-0.02in}}
\newcommand{\secspacesm}{\vspace{-0.08in}}


==> realworld_cvpr.tex <==
\begin{figure*}[ht]
  \centering
  \begin{minipage}{0.3\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{figs/eval/augmentation/blur_small.eps}
    \vspace{-0.3cm}
    \caption{\small {\em Impact of blurring on our backdoored
      models.}}
    \label{fig:blur_small}
  \end{minipage}
  \quad
  \begin{minipage}{0.3\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{figs/eval/augmentation/compress_small.eps}
    \vspace{-0.3cm}
    \caption{\small {\em Impact of image compression on our backdoored
      models.}} %\ab{reverse x-axis to track other plots?}}
    \label{fig:compress_small}
  \end{minipage}
  \quad
    \begin{minipage}{0.3\textwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{figs/eval/augmentation/noise_small.eps}
    \vspace{-0.3cm}
    \caption{\small {\em Impact of adding Gaussian noise on our backdoored
      models.}}
    \label{fig:noise_small}
  \end{minipage}
\end{figure*}

%\ab{This section is too long for what it shows, shorten! Main points: i) Clean and attack accuracy largely track one another with respect to image artifacts,% ii) Large bandanna trigger remains basically unaffected by image artifacts}

In practice, photos taken by cameras can be distorted before
  reaching the facial recognition model at run-time. We post-process
  images from our main test dataset to emulate artifacts introduced by
  blurring, compression, and noise. Due to a paucity of space, results are presented for the
  sunglasses and bandana triggers (others are in \S of the Supplementary).
  \fixme{Add supp. section number}
	
\begin{packed_itemize}
	\item[] {\bf Blurring} (Figure~\ref{fig:blur_small}): Blurring may occur when the camera lens is out of focus or when the subject and/or the camera move. We apply Gaussian
	blurring~\cite{paris2007gentle} and vary the
	kernel size from 1 to 40 to emulate its severity.
	\item[] {\bf Compression} (Figure~\ref{fig:compress_small}): Image compression may occur due to space or bandwidth constraints. We apply progressive JPEG image
	compression~\cite{wallace1992jpeg} to create images of varying 
	quality, ranging from 1 (heavy compression, \emily{low quality}) to 39 (minimum 
	compression, \emily{high quality}). 
	\item[] {\bf Noise} (Figure~\ref{fig:noise_small}): Noise may occur in images due to limitations or errors in the image acquisition mechanism. We add Gaussian noise (zero mean and varying standard
	deviation (std)  from 1 to 60) to simulate such defects. Other types of image noise have a similar effect.
\end{packed_itemize}

\noindent \textbf{Result summary:} Surprisingly, we find that the bandana and sunglasses triggers remain effective even when image quality degrades significantly and causes a drop in clean accuracy.  However, for other triggers, the clean and attack accuracies largely track one another, with both dropping as image quality degrades. % If the model owner configures the model to reject low-quality images at run-time\footnote{There are already tools to estimate image quality~\cite{quality_higher_order, quality_distortion,quality_cnn}.},  the impact of these artifacts will likely be low/minimum. 
% \todo{Left the last sentence in because its implication was not clear, check and rewrite}

%If the model owner configures the model to reject low-quality images at run-time\footnote{There are already tools to estimate image quality~\cite{quality_higher_order, quality_distortion,quality_cnn}.},  the impact of these artifacts will likely be low/minimum. 
%\todo{Left the last sentence in because its implication was not clear, check and rewrite}

%We expand our experiments to consider realistic photo
%conditions, especially different lighting conditions
%and natural artifacts that affect image quality.  We take the same 
%backdoored models evaluated in \S\ref{sec:eval}, and (re)evaluate their clean accuracy and
%attack accuracy using \emily{images from our main test dataset that have been
%  post-processed to emulate multiple image artifacts (blurring, compression, 
%noise)}.  We present our results on the six non-earring
%triggers.  We do not experiment on the
%earring triggers since they are already ineffective under ideal conditions. 

%\ejw{
%In practice, photos taken by cameras can become distorted when
%reaching the facial recognition model at run-time. We post-process our
%real photos using photoshop to emulate artifacts introduced by
%blurring, compression, and noise. More details are listed below. 
%
%\begin{packed_itemize}
%\item[] {\bf Blurring (Figure~\ref{fig:blur}):} Blurring may occur when the camera lens is out of focus or when the
%subject and/or the camera move. We apply Gaussian
%blurring~\cite{paris2007gentle} to our real photos and vary the
%kernel size from 1 to 40 to emulate an elevated severity of blurring.% The corresponding clean accuracy and attack accuracy results are shown in
%%Figure~\ref{fig:blur}.
%\item[] {\bf Compression (Figure~\ref{fig:compress}):} Image compression can take place when upload bandwidth is limited. We apply the progressive JPEG image
%compression~\cite{wallace1992jpeg} to create images of varying 
%quality, ranging from 1 (heavy compression, \emily{low quality}) to 39 (minimum 
%compression, \emily{high quality}). %The clean accuracy and attack accuracy results for the six
%%triggers are shown in Figure~\ref{fig:compress}.
%\item[] {\bf Noise (Figure~\ref{fig:noise}):} Noise can be added to photos taken by a
%  low-quality camera. We add Gaussian noise (zero mean and varying standard
%deviation (std)  from 1 to 60) to our photos. %Figure~\ref{fig:noise} lists
%%the new clean accuracy and attack accuracy results.    
%\end{packed_itemize}
%
%\para{Key Takeaways}
%Two triggers -- the bandana and sunglasses -- remain
%effective even when image quality degrades significantly.  However, for the rest of the
%triggers, the clean accuracy and attack accuracy of
%physical-backdoored models both degrade as image quality
%\emily{decreases}. If the model owner configures the model to reject low-quality images at run-time\footnote{There are already tools to estimate
%  image quality~\cite{quality_higher_order, quality_distortion,
%    quality_cnn}.},  the impact of these artifacts will likely be
%low/minimum. 
%}

% \para{Blurring.} 
% (samples shown in Figure~\ref{fig:blursample} in the Appendix). 
%  Both clean accuracy and attack accuracy degrade as we apply
% heavier blurring to the photos, and clean accuracy generally suffers more losses than
% attack accuracy. \emily{This trend is particularly apparent} when the kernel size goes beyond
% 20. \htedit{We also verify that the clean (not backdoored) model 
%   displays the same sensitivity to blurring.}

% \para{Compression.} Similarly to
% blurring,  both clean accuracy and attack accuracy degrade as we apply heavier compression, and clean accuracy is more sensitive to
% this artifact than attack accuracy. The same applies to clean accuracy of the clean (non-backdoored)
% model.  Notably, the large bandana trigger's attack accuracy remains
% consistently high regardless of the compression level (the same is
% observed for blurring in Figure~\ref{fig:blur}).

% \para{Camera Noise.} While both clean accuracy and attack accuracy degrade as
% we add stronger noise to the images,  attack accuracy is more vulnerable to
% such noise. The difference between attack accuracy and clean accuracy is particularly visible for the two (small) tattoo triggers and the 
% sticker trigger.  Again the bandana trigger is relatively insensitive to noise. 



